Impact-Robust Posture Optimization for Aerial Manipulation

We present a novel method for optimizing the posture of kinematically redundant torque-controlled robots to improve robustness during impacts. A rigid impact model is used as the basis for a configuration-dependent metric that quantifies the variation between pre- and post-impact velocities. By finding configurations (postures) that minimize the aforementioned metric, spikes in the robot's state and input commands can be significantly reduced during impacts, improving safety and robustness. The problem of identifying impact-robust postures is posed as a min-max optimization of the aforementioned metric. To overcome the real-time intractability of the problem, we reformulate it as a gradient-based motion task that iteratively guides the robot towards configurations that minimize the proposed metric. This task is embedded within a task-space inverse dynamics (TSID) whole-body controller, enabling seamless integration with other control objectives. The method is applied to a kinematically redundant aerial manipulator performing repeated point contact tasks. We test our method inside a realistic physics simulator and compare it with the nominal TSID. Our method leads to a reduction (up to 51% w.r.t. standard TSID) of post-impact spikes in the robot's configuration and successfully avoids actuator saturation. Moreover, we demonstrate the importance of kinematic redundancy for impact robustness using additional numerical simulations on a quadruped and a humanoid robot, resulting in up to 45% reduction of post-impact spikes in the robot's state w.r.t. nominal TSID.

==> approach.tex <==
\section{Our approach}
Now suppose that a robot is performing a task which involves an impact scenario. In such a scenario it is difficult to accurately plan or measure the forces applied on the robot during the impact. 

In this section, we will detail our approach for instantaneously optimizing the robot configuration wrt. to anticipated impacts (i.e impacts which are part of the task).  

First, we start our derivation from the general setting, that is not specific to impacts, where we consider the knowledge of the contact wrench in Eq.~(\ref{eq:realdyn}) to be uncertain. Accordingly, we rewrite the controller in Eq.~(\ref{eq:cntrl}), now as
\begin{equation}
   \bm{u} = \bm{G}^{-1}(\bm{M} \bnudt^{*} + \bm{h} - \bm{J}^{T}\bm{\hat{W}}_{\text{ext}})
   \label{eq:inacccntrl}
\end{equation}
The $\hat{}$ symbol represents evaluation of the external wrench at its nominal or measured value which in practice is not exactly equal to $\bm{W}_{\text{ext}}$. Consequently, the closed-loop acceleration which, in the ideal case, was stated in Eq~(\ref{eq:accFL}), now becomes 
\begin{equation}
        \bnudt = \bnudt^{*} + \bm{M}^{-1}(\q)\jacob^{T} \Delta\bm{W}_{\text{ext}}
    \label{eq:CLdyn}
\end{equation}
Where $\bm{\Delta}\bm{W}_{\text{ext}}$ is the difference between the nominal and the real external wrench. 
We can rewrite in Eq~(\ref{eq:CLdyn}) as follows
\begin{equation}
    \Delta \bnudt = \bm{M}^{-1}(\q)\jacob^{T} \Delta\bm{W}_{\text{ext}}
    \label{impact_sens}
\end{equation} 
Where $\Delta \bnudt = \bnudt - \bnudt^{*}$. Equation~(\ref{impact_sens}), represents the instantaneous sensitivity of the closed-loop acceleration (in closed-form) to the mismatch in the external wrench, which we denote as $\bm{\Gamma}(t)$
\begin{equation}
    \label{eq:Gamma}
    \bm{\Gamma}(t) = \bm{M}^{-1}(\q)\jacob^{T}
\end{equation}
Suppose $\Delta\bm{W}_{\text{ext}} \in \mathcal{W}$ where $\mathcal{W}$ represents the set of all possible perturbations around the nominal wrench. We then define the set $\mathcal{Y} = \{ \bnudt^{*} + \bm{M}^{-1}(q)\jacob^{T} \Delta\bm{W}_{\text{ext}}, \forall \Delta\bm{W}_{\text{ext}} \in \mathcal{W}  \}$ 


Suppose we can define an ellipsoid in the perturbed parameter space, where the kernel matrix contains the bounds on the parameter deviation. 
\begin{equation}
     \Delta\bm{W}_{\text{ext}}^{T} \bm{W}^{-1}_\gamma \Delta\bm{W}_{\text{ext}} = 1
    \label{eq:paramellipsoid}
\end{equation}
Consequently we project the ellipsoid in the perturbed parameter space into the acceleration space. and we get 
\begin{equation}
    \Delta \dot{\bm{\nu}}^{T} (\bm{\Gamma} \bm{W}_\gamma  \bm{\Gamma}^{T})^{\dagger} \Delta \dot{\bm{\nu}} = 1
    \label{eq:accellipsoid}
\end{equation}

We pose the following question, can we exploit the robot's kinematic redundancy to design a virtual input $\dot{\bm{\nu}}^{*}$ which minimizes a suitable norm of the quantity $\bm{\Gamma}(t)$. One possible choice is the Frobenius norm of of the matrix $H_{\Gamma} = (\bm{\Gamma} \bm{W}_\gamma  \bm{\Gamma}^{T})$ which represents the worst case deviation or axis of the perturbed acceleration space. if $\bm{\Gamma}(t)$ is a function of the robots configuration $\bm{q}$, then we exploit the robot's kinematic redundancy and attempt to minimize the Frobenius norm $|| H_{\Gamma} ||_{F}$ in the null space of the task Jacobian. This is done as follows
\begin{equation} 
    \bm{\dot{\nu}}_{\text{null}} =  - \bm{K} \nabla_{\bm{q}} || H_{\Gamma} ||_{F} - \bm{K}_d \bm{\nu}
\end{equation}
Where $\bm{K}$ is a tunable positive definite gain matrix and $- \bm{K}_d \bm{\nu}$ represents the damping necessary to stabilize the null space dynamics.




At this point we

Now we ask ourselves what are the practical consequences of this mismatch in accounting for external generalized forces. To answer this question lets first consider the nominal case, where our controller successfully linearize the system to achieve Eq.~(\ref{eq:accFL}) and the robot is accurately tracking the reference trajectory. It is also reasonable to consider that nominally, that $\bnudt_{t}^{*}$.

Suppose we can define an ellipsoid in the perturbed parameter space, where the kernel matrix contains the bounds on the parameter deviation. 
\begin{equation}
     \Delta\bm{W}_{\text{ext}}^{T} \bm{W}^{-1}_\gamma \Delta\bm{W}_{\text{ext}} = 1
    \label{eq:paramellipsoid}
\end{equation}
Consequently we project the ellipsoid in the perturbed parameter space into the acceleration space. and we get 
\begin{equation}
    \Delta \dot{\bm{\nu}}^{T} (\bm{\Gamma} \bm{W}_\gamma  \bm{\Gamma}^{T})^{\dagger} \Delta \dot{\bm{\nu}} = 1
    \label{eq:accellipsoid}
\end{equation}

We pose the following question, can we exploit the robot's kinematic redundancy to design a virtual input $\dot{\bm{\nu}}^{*}$ which minimizes a suitable norm of the quantity $\bm{\Gamma}(t)$. One possible choice is the Frobenius norm of of the matrix $H_{\Gamma} = (\bm{\Gamma} \bm{W}_\gamma  \bm{\Gamma}^{T})$ which represents the worst case deviation or axis of the perturbed acceleration space. if $\bm{\Gamma}(t)$ is a function of the robots configuration $\bm{q}$, then we exploit the robot's kinematic redundancy and attempt to minimize the Frobenius norm $|| H_{\Gamma} ||_{F}$ in the null space of the task Jacobian. This is done as follows
\begin{equation} 
    \bm{\dot{\nu}}_{\text{null}} =  - \bm{K} \nabla_{\bm{q}} || H_{\Gamma} ||_{F} - \bm{K}_d \bm{\nu}
\end{equation}
Where $\bm{K}$ is a tunable positive definite gain matrix and $- \bm{K}_d \bm{\nu}$ represents the damping necessary to stabilize the null space dynamics.


==> formulation.tex <==
\section{Closed loop state sensitivity}
In this section a very brief account of the closed loop sensitivity metric is given for the purpose of keeping the report self contained. In the case that the reader requires more information please read the cited references. 

The closed loop state sensitivity that we denote as $\Pi$ has been introduced in \cite{2018f-RobDelFra} and extended in \cite{brault2021robust}. In these works a paramterized trajectory was optimized offline. The objective of the optimization was to minimize the frobenius norm of $\Pi$. 

Another more expressive norm for $\Pi$ was proposed by Paolo Robuffo Giordano. The norm used is the p-norm of $\Pi$ which is a smooth approximation of maximum eigenvalue of the following matrix 

\begin{equation}
    \lambda_{max}  = (eig(\Pi^{T}W\Pi))
\end{equation}

where $W$ is a matrix that incorporates knowledge of the range of parameter uncertainty. 

The detailed explanation of p-norm of $\Pi$ and related quantities, can be found in the appendix. 

As explained in \cite{2018f-RobDelFra}, \cite{brault2021robust} , $\Pi$ does not, in general, have a closed form solution. However, the evolution of $\Pi$ can be derived quite easily as shown below. 

\begin{equation}
    \Dot{\Pi} = F \Pi + D
\end{equation}

The derivation $F$ and $D$ can be found in \cite{brault2021robust}. The important thing to note is that they are composed of partial derivatives of the system dynamics and the controller dynamics with respect to state variables, control variables, and model parameters. 


\section{Aerial Manipulator dynamics \& Contol}

We consider an aerial robotic system composed of a \emph{fully actuated aerial vehicle} endowed with a \emph{robotic arm} possessing $n_{a}$ Degrees of Freedom (DoFs). We shall refer to the full system as an \emph{aerial manipulator} (AM), see Fig.~\ref{fig:aerial_manip} for an example. 

The configuration of the AM is given by $\configSpaceElem = (\posb, \phi_{b}, \jointPos) \in \configSpace \subseteq \mathbb{R}^3 \times \mathbb{R}^3 \times \mathbb{R}^{n_{a}}$. Where, $\posb \in \mathbb{R}^3 $ and $\phi_{b} \in \mathbb{R}^3 $ represent the position and orientation (in roll-pitch-yaw minimal orientation representation) of the flying base frame with respect to world frame, respectively, and $\jointPos\in \mathbb{R}^{n_{a}}$ represents the arm joint angles.

\subsection{System dynamics}

In \cite{lippiello2012cartesian} the detailed derivation of the dynamic model of the system can be found, which is based on euler lagrange formalism.

The system dynamics can be written in the form

\begin{IEEEeqnarray}{LCL}
    \label{eq:system_dynamics}
    \inertia(q)\dot{\nu} + \coriolis(q,\nu) + \gravity(q) = \begin{bmatrix} \propellerWrench^\top \torqueArm^\top \end{bmatrix}^\top
\end{IEEEeqnarray}
%
where $\inertia(\configSpaceElem) \in \mathbb{R}^{(6+n_{a})\times(6+n_{a})}$ is the inertia matrix, $\coriolis(\configSpaceElem,\dconfigSpaceElem) \in \mathbb{R}^{6+n_{a}}$ represents the Coriolis and centrifugal effects, and $\gravity(\configSpaceElem) \in \mathbb{R}^{6+n_{a}}$ is the gravity vector. 

The control wrench is represented by $\begin{bmatrix} \propellerWrench^\top \torqueArm^\top \end{bmatrix}^\top$ where $\propellerWrench \in \mathbb{R}^6$ is the control wrench applied by/on the aerial vehicle, and $\torqueArm \in \mathbb{R}^{3}$ represents the input torques of the $n_a$-DoF arm. 

The actual system inputs of the aerial vehicle are the individual propeller thrust forces which can be related linearly to the squares of the propeller angular rates denoted with $\propellerSquares\in \mathbb{R}^{n_{p}}$, where $n_{p}$ is the number of propellers. The wrench mapping between $\propellerWrench$ and $\propellerSquares$ is given by a grasp-like matrix $\matr{G}_w \in \mathbb{R}^{6\times n_p}$, i.e.,
%
\begin{IEEEeqnarray}{LCL}
    \label{eq:system_alloc}
    \propellerWrench = \matr{G}_w \propellerSquares.
\end{IEEEeqnarray}
%

The matrix $\matr{G}_w$ is composed of geometric parameters and aerodynamic parameters

\begin{itemize}
    \item The angles of tilt of the propeller $\alpha$ and $\beta$
    \item The distance $l_{rod}$ between the propellers and the CoM of the UAV
    \item $k_f$ and $k_d$, which are the coefficients of thrust and drag, respectively
\end{itemize}

\subsection{Operational Space Control}

The task for a manipulator is usually defined in terms of the End Effector EE. In the following we will consider a full pose trajectory tracking task for the EE (task dimension = 6). 

The controller presented in this section follows the same approach presented in \cite{RYLL2018138}, however here we correct some mistakes that were found in \cite{RYLL2018138}. Therefore we present the controller in details. 

In the following the subscript $pc$ will be used to distinguish the quantities used in the controller from their real values. 

The position and the orientation of EE frame with respect to the world can be computed in terms of $\configSpaceElem$ using the Denavit-Hartenberg paramterization, and 
the differential kinematics can be used then to compute the EE instantaneous velocities $\EEgenVel = [\velEE^\top \vSpace \omegaEE^\top]^\top \in \mathbb{R}^{6}$ as
%
\begin{IEEEeqnarray}{LCL}
    \label{eq:system_kin1}
    \EEgenVel = \Jacob \dconfigSpaceElem,
\end{IEEEeqnarray}
%
where $\Jacob$ is the geometric Jacobian. Furthermore, the acceleration level differential kinematics, which is relevant to our proposed control scheme, is computed by taking the time derivative of (\ref{eq:system_kin1})
%
\begin{IEEEeqnarray}{LCL}
    \label{eq:system_kin2}
    \EEgenAcc = \Jacob \dot{\nu} + \JacobDot \nu.
\end{IEEEeqnarray}
%

\subsubsection{Camputing a Virtual input at the EE acceleration level}

The operational space controller is acceleration based. This means that a virtual input designed at the acceleration level for the end effector, which is composed of PD + feedforward term  as follows:

\begin{align}
\vect{a}_{e_1}
=
\ddot{\vect{p}}^r_e
+
\matr{K}_{P_1}(\dot{\vect{p}}^r_e-\dot{\vect{p}}_e) + \matr{K}_{P_2}(\vect{p}^r_e-\vect{p}_e)
\label{eq:posinput}
\end{align}
\begin{align}
\vect{a}_{e_2}
=
\dot{\vect{\omega}}^r_e + \matr{K}_{\omega_1}(\vect{\omega}^r_e-\vect{\omega}_e) + \matr{K}_{\omega_2}\vect{e}_R
\label{eq:rotinput}
\end{align}
with the orientation error defined as
\begin{equation}
\vect{e}_R=\frac{1}{2}[\matr{R}_e^T \matr{R}_e^r-\matr{R}_e^{r^{T}} \matr{R}_e]_\vee.
\label{eq:roterror}
\end{equation}

The virtual input is changed from the operational space to the joint space by the inverse differential kinematics defined at the acceleration level. Additionally, the proposed system, we have $n_a$ redundant degrees of freedom that be use to optimize additional criteria. This can be done by projecting our preferred joint $a_z$ accelerations in the null space of the task. 

\begin{align}
\vect{a}_q
=
\WeightJacobInv (\vect{a}_e-\JacobDot \dconfigSpaceElem \big)
+
\big(
\matr{I}_{6+n_a}-\WeightJacobInv 
\matr{J}(\configSpaceElem)
\big)
\vect{a}_z,
\label{eq:invKinematics}
\end{align}

\subsubsection{Redundancy resolution \& the optimization of $\Pi$ }

To design $\vect{a}_z$ we use the projected gradient approach~\cite{redund}, in which  desired behaviors are represented as optimization criteria of some objective functions. The weighted sum of the gradients of these functions is then projected in the null space using~\eqref{eq:invKinematics}.  A term that stabilizes the internal dynamics is also added to $\vect{a}_z$ by default.

In general, to keep a variable $x$ as close as possible to the midpoint of its operating range $x \in\left[x_{l}, x_{u}\right]$ the following objective function can be used 
\begin{equation}
H_{\text {r}}(x)=\frac{1}{2} \left(\frac{x-\bar{x}}{x_{u}-x_{l}}\right)^{2},
\label{eq:obj_range}
\end{equation}
where $\overline{x}=\frac{x_{u}+x_{l}}{2}$.

As discussed in~\cite{RYLL2018138}, for a uni-directional thrust fully actuated aerial vehicle -- i.e., the typical aerial vehicle possess propellers that can produce force in only one direction -- it is important to keep the platform tilt angles (i.e., the roll and pitch) within an operating range to avoid generating unfeasible  thrust commands. Consequently, we use two objective functions similar to~\eqref{eq:obj_range} -- namely $H_{\text{r}}(\phi)$ and $H_{\text{r}}(\theta)$ where $\phi$ and $\theta$ are the roll and pitch angles respectively extracted from $\rotb$ -- to favor configurations with tilt angles that are close to zero. Similarly, we use $H_{\text{r}}(\jointPosi)$ to favor configurations in which the $i^{th}$ joint angle of the arm within is in the middle of its range, for all $i = 1, \ldots, n_a$. Finally, $a_{z}$ is computed as follows
\begin{equation}
    \vect{a}_z =  \frac{1}{2 + n_a} \nabla H - \matr{K}_{n}\dconfigSpaceElem
\label{PG_null}
\end{equation}
\begin{equation*}
\nabla H =\left( -k_1\nabla_\phi  H_{\text{r}}(\phi) - k_2\nabla_\theta H_{\text{r}}(\theta) - \sum_{i=1}^{n_a} k_i\nabla_{\jointPosi} H_{\text{r}}(\jointPosi)\right)
\end{equation*}
where, $\matr{K}_n \in \mathbb{R}^{(6+ n_a)\times(6+ n_a)}$ is a positive definite diagonal matrix, and $k_1$, $k_2$, and the $k_i$'s are positive scalar gains that define a priority between the gradients.

Additionally we would like to use the fact the robot is kinematically redundant in order to optimize $\Pi$. In particular we would like to minimize the p-norm of $\Pi$. lets denote that cost function as $H(\Pi)$. Consequently, following the projected gradient approach we can extend equation \ref{PG_null} by adding the gradient of p-norm cost function $\nabla H(\Pi)$ 

\begin{equation}
    \vect{a}_z =  \frac{1}{2 + n_a} \nabla H - \matr{K}_{\pi} 
 \nabla_{q} H(\Pi) - \matr{K}_{n}\dconfigSpaceElem
\label{PG_null_pi}
\end{equation}

Similarly to $\Pi$, the gradient of $\Pi$ does not have a closed form solution but its dynamics can be derived as shown in \cite{brault2021robust}. Alternatively, one can obtain the gradient of $\Pi$ numerically by finite differences with the formula shown below.

\begin{equation}
    \nabla f(\theta) = \frac{f(\theta + \epsilon) - f(\theta - \epsilon)}{2\epsilon}
\end{equation}


In this work, we use the finite differences approach for computing the gradients. The motivation is that since we are considering highly dimensional redundant robotic systems such as aerial manipulators, the analytical computation of the gradient dynamics is computationally very expensive. We will demonstrate that using the numerically obtained gradients is indeed effective in minimizing the sensitivity and computational feasible for the real-time control constraint. 

\subsubsection{Computing system inputs via inverse dynamics}

Finally, inverse dynamics are used in order to compute the required inputs as shown below. 

\begin{equation}
    \label{eq:inv_dynamics}
      \begin{bmatrix} \propellerSquares \\ \torqueArm \end{bmatrix} = \begin{bmatrix} \matr{G}_{wpc} & 0_{6xna} \\
       0_{nax6} & I_{na} \end{bmatrix}^{-1} (\inertia_{pc}(\configSpaceElem)a_{q} + \coriolis_{pc}(\configSpaceElem,\dconfigSpaceElem) + \gravity_{pc}(\configSpaceElem)) 
\end{equation}
%

==> prelim.tex <==
\section{Background}\label{sec:prelim}
In this section, we introduce the preliminaries required to describe our approach. We will focus on floating base kinematically redundant robots when describing a robot's configuration, however our approach is also valid for fixed base kinematically redundant robots. 

\subsection{Operational space control}
The Operational space control formulation, also referred to as task space control, was first proposed in \cite{1087068}. This formulation presents a general approach to control a robot's task space, for example, controlling the pose of an End Effector (EE) of a robotic arm. In the following we summarize the approach, which is fundamental in our further developments.

Consider the following task kinematics described at the acceleration level
\begin{equation}
    \bnudt_t = \jacob \bnudt + \jacobdt
    \label{eq:task_kin}
\end{equation}
where, $\q$ represents the robot's configuration space $\mathbb{Q} \subset \mathbb{SE}(3) \times \mathbb{R}^{n_j}$, which comprises of the floating base full pose in addition to $n_j$ joints. $\bnudt \in \mathbb{R}^{n_j + 6}$ represents the robot's acceleration in the configuration space, while $\bnudt_t \in \mathbb{R}^{n_t}$ represents the robot's task space accelerations. We are interested in robot's that are kinematically redundant i.e $n_j > n_t$. Note that for under-actuated robots such as a humanoid robot, Eq.~(\ref{eq:task_kin}) can be rewritten highlighting the actuated and not actuated joints in two separate terms (see for example REF). In order to simplify the next mathematical developments, we will assume that that all $\bnudt$ are actuated, however our approach is not restricted to fully actuated robots as we will demonstrate in the subsequent sections.   

Suppose, we would like to impose an acceleration $\bnudt_{t}^{*}$ to the robot task space, where  $\bnudt_{t}^{*}$ represents a virtual control input, for example a proportional and damping controller (PD controller) and a feed-forward acceleration.
\begin{equation}
    \bnudt_{t}^{*} = \bnudt_{t}^{\text{ff}} + \bm{K}_{p}\bm{e}_p + \bm{K}_{v}\bm{e}_v
    \label{main_task}
\end{equation}
One can then compute the corresponding joint space accelerations 
\begin{equation}
    \bnudt^{*} = \jacob_{W}^{\dagger}(\bnudt_{t}^{*} - \jacobdt + \bm{P}(\bm{q})\bnudt_{\text{null}}
    \label{eq:invdiffKin}
\end{equation}
where $\jacob_{W}^{\dagger}$ represents a weighted Moore-Penrose inverse, while $\bm{P}(\bm{q})$ represents the null space projector and $\bnudt_{\text{null}}$ is a preferred acceleration to be projected in the null-space of the task and acts as a secondary task. It is also possible to have a hierarchy of tasks defined with a strict priority and use successive null space projections to achieve them. Generally, a task is composed of some 

Consider the following representation of the dynamics of a floating-base robotic system
\begin{equation}
    \bm{M}(\q) \bnudt + \bm{h}(\q,\bnu) = \bm{G}\ip + \jacob^{T}\bm{W}_{\text{ext}}
    \label{eq:realdyn}
\end{equation}
Assuming perfect knowledge of the robot model in Eq.~(\ref{eq:realdyn}), we can then design a static feedback linearization scheme as follows  (removing the dependency on the state for compactness)
\begin{equation}
   \ip = \bm{G}^{-1}(\bm{M} \bnudt^{*} + \bm{h} - \bm{J}^{T}\bm{W}_{\text{ext}})
   \label{eq:cntrl}
\end{equation} 
The controller in Eq.~(\ref{eq:cntrl}) will linearize the dynamics and imposes the following equality
\begin{equation}
    \bnudt = \bnudt^{*}
    \label{eq:accFL}
\end{equation}


\subsection{Task Space Inverse Dynamics}

In order to take into account the robot's physical limits, such as the actuator limits and joint limits, we can formulate the operational space controller as a quadratic program with hard constraints. 

\begin{equation}
\begin{aligned}
\min_{\bm{u},\bm{\dot{\nu}}} \quad & (\bm{\dot{\nu}} - \bm{\dot{\nu}}_{\text{null}})^{T} \bm{W} (\bm{\dot{\nu}} - \bm{\dot{\nu}}_{\text{null}})\\
\textrm{s.t.} \quad & \bm{M} \bm{\dot{\nu}} + \bm{h} = \bm{G}\bm{u} + \bm{W}_{\text{ext}} \\
  & \bm{\dot{\nu}}_{t}^{*} =  \bm{J}(\bm{q})\bm{\dot{\nu}} + \dot{\bm{J}}(\bm{q})\bm{\nu} \\
  &  \underline{\bm{{u}}} \leq \bm{u} \leq \overline{\bm{{u}}}    \\
  &  \underline{\bm{{\dot{\nu}}}} \leq \bm{\dot{\nu}} \leq \overline{\bm{{\dot{\nu}}}}    \\
\end{aligned}
\end{equation}

\subsection{Controller sensitivity to Impacts}
The effects of impact on robots have been studied extensively in the literature and some approaches have been proposed to tackle impact in a proper way, examples include reference spreading \cite{9867812} and impact invariant control \cite{9636094}. 


==> results.tex <==
\section{Results}
Some snapshots of the results. Work in progress
\begin{figure*}[t!]
    \centering
    \includegraphics[scale=0.3]{figures/before_after_AM.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure*}

\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.15]{figures/qp_hum_before_after.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}



==> symbol_def_old.tex <==
% ---------- Standard Commands ------------------
\usepackage{color}
\newcommand\red[1]{{\textcolor{red}{#1}}}
\newcommand\blue[1]{{\textcolor{blue}{#1}}}
\newcommand\green[1]{{\textcolor{green}{#1}}}

%% Help full working commands
\newcommand\sectionDetails[2]{\red{*** Section by \textbf{#1}, ideal length #2 columns *** \newline}}
\newenvironment{partDetails}[1]
    {\noindent \red{------ Start part by \textbf{{#1}} ------}
    }
    {\noindent \red{------ End part ------}
    }

% --------- References ----------------------
\newcommand{\fig}{Fig.~}	 % figure ref
\newcommand{\eqn}{Eq.~}	     % equation ref
\newcommand\gabrisays[1]{\textcolor{red}{#1}} % comments from gabri


% ---------- New commands ------------------
\newcommand{\vect}[1]{\bm{#1}}		   % vectors
\newcommand{\matr}[1]{\bm{#1}}		   % matrices
\renewcommand{\skew}[1]{\matr{S}(#1)}  % skew operator
\newcommand{\frameV}{\mathcal{F}}	   % generic frame

\newcommand{\origin}{O}						% origin
\newcommand{\vX}{\vect{x}}					% x-axis
\newcommand{\vY}{\vect{y}}					% y-axis
\newcommand{\vZ}{\vect{z}}					% z-axis
\newcommand{\vE}[1]{\vect{e}_{#1}}			% standard unit axis

\newcommand{\eye}[1]{\matr{I}_{#1}}


% --------- Spaces, Groups and Frames ----------------------
\newcommand{\configSpace}{\mathcal{Q}}            % configuration space
\newcommand{\configSpaceElem}{\vect{q}}           % configuration space element
\newcommand{\dconfigSpaceElem}{\vect{\dot{q}}}          % derivative configuration space element
\newcommand{\ddconfigSpaceElem}{\vect{\ddot{q}}}   % sec. derivative configuration space
\newcommand{\frameW}{\frameV_W}			% world frame
\newcommand{\originW}{\origin_W}		% origin world frame
\newcommand{\xW}{\vX_W}				% x-axis world frame
\newcommand{\yW}{\vY_W}				% y-axis world frame
\newcommand{\zW}{\vZ_W}				% z-axis world frame

\newcommand{\frameb}{\frameV_b}      	          % base frame
\newcommand{\originb}{O_{b}}					% origin robot frame
\newcommand{\xb}{\vX_{b}}								% x-axis robot frame
\newcommand{\yb}{\vY_{b}}								% y-axis robot frame
\newcommand{\zb}{\vZ_{b}}								% z-axis robot frame

\newcommand{\frameE}{\frameV_E}          	      % EE frame
\newcommand{\originE}{O_{E}}					% EE robot frame
\newcommand{\xE}{\vX_{E}}								% x-axis EE frame
\newcommand{\yE}{\vY_{E}}								% y-axis EE frame
\newcommand{\zE}{\vZ_{E}}								% z-axis EE frame


% --------- Drone ----------------------
\newcommand{\posb}{\vect{p}_b}          % base position
\newcommand{\rotb}{\matr{R}_b}          % base rotation
\newcommand{\velb}{\vect{v}_b}          % base linear velocity
\newcommand{\omegab}{\vect{\omega}_b}   % base angular velocity
\newcommand{\drotb}{\dot{\matr{R}}_b}   % base rotation derivative


% --------- Robotic arm ----------------------
\newcommand{\numJoints}{n}                   % number of joints
\newcommand{\jointPos}{\vect{q}_A} % joints position
\newcommand{\jointPosi}{\vect{q}_{A_{i}}}
\newcommand{\jointVel}{\vect{v}_A}           % joints velocity
\newcommand{\torqueArm}{\vect{\tau}_A} % joints torque
\newcommand{\EEgenVel}{\vect{\dot{x}}_E}
\newcommand{\EEgenAcc}{\vect{\ddot{x}}_E}
\newcommand{\velEE}{\vect{v}_E}              % end eff linear velocity
\newcommand{\omegaEE}{\vect{\omega}_E}       % end eff angular velocity
\newcommand{\rotationMapping}{\matr{\bar{R}}}      % rotation mapping for EE twist
\newcommand{\rotE}{\matr{R}_{E}} % EE rotation
\newcommand{\Jacob}{\matr{J_{pc}}(\configSpaceElem)} % contact Jacobian (constrained dir)
\newcommand{\WeightJacobInv}{\matr{J}_W^\dagger(\configSpaceElem)} 
\newcommand{\JacobDot}{\matr{\dot{J_{pc}}}(\configSpaceElem,\dconfigSpaceElem)}     % contact 
\newcommand{\dcontactJacobConstr}{\dot{\matr{J}}_E^c}     % contact Jacobian derivative (constrained dir)
\newcommand{\contactJacobFree}{\matr{J}_E^f}       % contact Jacobian (free dir)
\newcommand{\contactJacobConstrTransp}{\matr{J}_E^{c\top}}     % contact Jacobian transp (constrained dir)
\newcommand{\contactJacobFreeTransp}{\matr{J}_E^{f\top}}       % contact Jacobian transp (free dir)
\newcommand{\fConstr}{\vect{f}_{c}}      % contact forces
\newcommand{\fViscous}{\vect{f}_{f}}    % viscous friction forces
\newcommand{\contactJacobFreeDot }{\matr{\dot{J}}_E^f}

% --------- Dynamics ----------------------
\newcommand{\inertia}{\matr{M}}		          % inertial matrix
\newcommand{\coriolis}{\vect{c}}              % Coriolis
\newcommand{\gravity}{\vect{g}}	     	      % gravity
\newcommand{\propellerWrench}{\vect{w}_b} % propellers wrench
\newcommand{\contactWrench}{\vect{w}_{\rm ext}}     % contact wrench
\newcommand{\humanWrench}{\vect{w}_{h}}     % human wrench
\newcommand{\propellerSquares}{\vect{w}_{p}}     % squares of the propeller rates
\newcommand{\contactJacob}{\matr{J}_E}        % contact Jacobian
\newcommand{\contactActivation}{\beta}        % contact activation parameter
\newcommand{\propMapping}{\matr{G}_w}         % propellers mapping
\newcommand{\propMappingForce}{\matr{G}_{w1}}         % propellers mapping
\newcommand{\propMappingMoment}{\matr{G}_{w2}}         % propellers mapping
\newcommand{\omegaProp}{\vect{\omega}_P}      % propellers square ang. vel.
\newcommand{\dcontactJacob}{\dot{\matr{J}}_E} % contact Jacobian derivative
\newcommand{\inputAllocation}{\matr{G}}
\newcommand{\inpt}{\vect{u}}


% --------- Controller ----------------------
\newcommand{\outp}[1]{{y}_{#1}}
\newcommand{\relDegree}[1]{{(r_{#1})}}
\newcommand{\outps}{\vect{y}}
\newcommand{\outpsDes}{\vect{y}^d}
\newcommand{\numOutp}{m}
\newcommand{\regMatrix}{\matr{D_{\regularization}}}

% --------- QP Optimization ----------------------
\DeclareMathOperator*{\minimize}{minimize}
\newcommand{\inputControl}{\vect{u}}     % control input
\newcommand{\inputControlExtended}{\vect{u}'}     % control input
\newcommand{\accStack}{\vect{a}}         % all tasks accelerations
\newcommand{\accStackCtrl}{\vect{a}^\star}         % all tasks accelerations
\newcommand{\weightTask}{\matr{W}_{u_{q}}}     % weights all tasks weights
\newcommand{\biasVectContact}{\vect{b}}       % bias vector constraints
\newcommand{\contactStabilityMatr}{\matr{C}}  % constraint matrix
\newcommand{\upperBoundU}{\inputControl_u}  % upper bound u
\newcommand{\lowerBoundU}{\inputControl_l}  % lower bound u
\newcommand{\dvelEE}{\dot{\vect{v}}_E}          % end eff linear acc
\newcommand{\domegaEE}{\dot{\vect{\omega}}_E}   % end eff angular acc
\newcommand{\dvelR}{\dot{\vect{v}}_R}           % base linear acc
\newcommand{\domegaR}{\dot{\vect{\omega}}_R}    % base angular acc
\newcommand{\regularization}{\vect{r}_a}    % regularization
\newcommand{\jointAcc}{\dot{\vect{v}}_A}          % joints acc
\newcommand{\multiplInput}{\matr{H}(\configSpaceElem)}        % control input multiplier QP
\newcommand{\biasQP}{\vect{h}(\configSpaceElem,\dconfigSpaceElem)}              % bias QP
\newcommand{\EEfreeAcc}{\dot{\vect{v}}_f}   % EE free acc
\newcommand{\nTasks}{n_t}        % number of takss
\newcommand{\numPropellers}{p}   % number of propellers
\newcommand{\nInput}{ \numJoints + \numPropellers + \numConstraints}   % number of inputs
\newcommand{\rank}{\text{rank}}  % matrix rank

%% Gains
\newcommand{\gainDR}{\matr{K}_{DR}}  % gain D base pos
\newcommand{\gainPR}{\matr{K}_{PR}}  % gain D base pos
\newcommand{\gainDRw}{\matr{K}_{DR\omega}}  % gain D base rot
\newcommand{\gainPRw}{\matr{K}_{PR\omega}}  % gain P base rot
\newcommand{\gainDA}{\matr{K}_{DA}}  % gain D joints
\newcommand{\gainPA}{\matr{K}_{PA}}  % gain P joints
\newcommand{\gainDF}{\matr{K}_{DF}}  % gain D EE
\newcommand{\gainPF}{\matr{K}_{PF}}  % gain P EE
\newcommand{\gainIC}{\matr{K}_{IC}}  % gain I force
\newcommand{\gainPC}{\matr{K}_{PC}}  % gain I force
\newcommand{\EEfreeVel}{\vect{v}_f}
\newcommand{\EEfreePos}{\vect{p}_f}
\newcommand{\rotError}{\vect{e}_{R\omega}}

%%%% OLD COMMANDS %%%%

% --------- References ----------------------

\newcommand{\tab}{Tab.~}	    % table ref
\newcommand{\cha}{Chap.~}	    % chapter ref
\newcommand{\sect}{Sec.~}	    % section ref
\newcommand{\prob}{Problem~}	% problem ref
\newcommand{\scenario}[1]{Scenario~{#1})}
\newcommand{\SO}[1]{SO({#1})}   % orthogonal group
\newcommand{\nR}[1]{\mathbb{R}^{#1}}   % real number
\newcommand{\vSpace}{\;\,}
\newcommand{\nN}[1]{\mathbb{N}^{#1}}   % integer number



==> theory.tex <==
\section{Instantaneous Sensitivity to Contact Uncertainty}
Consider the following Euler-Lagrange representation for the dynamics of a fully-actuated robot
\begin{equation}
    \bm{M}(\q) \bnudt + \bm{h}(\q,\bnu) = \bm{G}\ip + \jacob^{T}\bm{W}_{\text{ext}}
    \label{eq:realdyn}
\end{equation}
where, $\q$ represents the robot's configuration space $\in \mathbb{R}^{n_j}$ which comprises of the $n_j$ joints.

Due to the full actuation of the system, it can be controlled by a static feedback linearization scheme. The controller, which is presented in Eq.~(\ref{eq:cntrl}) (removing the dependency on the state for compactness), uses estimates of the system dynamics 
\begin{equation}
   \ip = \bm{G}^{-1}(\hat{\bm{M}} \bnudt^{*} + \hat{\bm{h}} - \hat{\bm{J}}^{T}\hat{\bm{W}}_{\text{ext}})
   \label{eq:cntrl}
\end{equation} 
Where $\bnudt^{*} \in \mathbb{R}^{n_j}$ is the desired robot acceleration to be imposed i.e $\bnudt = \bnudt^{*}$. It represents a virtual input that is often comprised of a proportional and damping feedback action in addition to a feed-forward acceleration. The $\hat{}$ symbol represents evaluation of the dynamics at their nominal or estimated values. In the following arguments, we will assume that controller has access to accurate estimates of the dynamic quantities with the exception of the external wrench such that $\hat{\bm{M}} = \bm{M}$, $\hat{\bm{h}} = \bm{h}$, and $\hat{\bm{J}} = \bm{J}$, therefore in the absence of generalized contact forces $\bm{W}_{\text{ext}} = \hat{\bm{W}}_{\text{ext}} = \bm{0}$, the controller in Eq.~(\ref{eq:cntrl}) will successfully linearize the system and imposes the desired acceleration. The limitation of the assumption that the controller has access to perfect knowledge of the system's dynamic parameters will be analyzed empirically in the sec.\amr{num}.

Now consider a situation where the robot is in contact with the environment such that $\bm{W}_{\text{ext}} \neq \bm{0}$. Moreover, the controller does not have access to an accurate estimate of the external wrench i.e $\hat{\bm{W}}_{\text{ext}} \neq \bm{W}_{\text{ext}}$. Consequently, the resulting instantaneous closed-loop acceleration will take the form
\begin{equation}
        \bnudt = \bnudt^{*} + \bm{M}^{-1}(\q)\jacob^{T} \Delta \bm{w}_{e}
    \label{eq:CLdyn}
\end{equation}
Where $\Delta\bm{w}_{e}$ is the difference between the nominal and the real external wrench. 
We can rewrite in Eq~(\ref{eq:CLdyn}) as follows
\begin{equation}
    \Delta \bnudt = \bm{M}^{-1}(\q)\jacob^{T} \Delta\bm{w}_{e}
    \label{impact_sens}
\end{equation} 
Where $\Delta \bnudt = \bnudt - \bnudt^{*}$. Equation~(\ref{impact_sens}), represents the instantaneous sensitivity of the closed-loop acceleration (in closed-form) to the mismatch in the external wrench, which we denote as $\bm{\Gamma}(q)$
\begin{equation}
    \label{eq:Gamma}
    \bm{\Gamma}(q) = \bm{M}^{-1}(\q)\jacob^{T}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Optimizing for Impact Insensitivity}
Impact events represent contacts that happen at non-zero speed and constitute a significant change of momentum for the impacting bodies over a short period of time, ex. milliseconds. During an impact event, it is difficult to precisely estimate or measure the impact forces. Estimators, as in [residual], have their own dynamics and delay in estimating forces, while forces sensors suffer from bias, hysteresis and noise, which might be amplified during an impact. In this case, there will be a mismatch between the actual impact forces and their estimate within the controller equations, leading to variations of the system's acceleration from their nominal values as described in Eq.~(\ref{impact_sens}). Potentially, large uncertainties can lead to instantaneously large variations or spikes in the robot accelerations and consequently lead to spikes in the control effort. With that in mind, it is particularly useful to design a control strategy that renders the robot insensitive to impacts, i.e the uncertainty in the impact forces does not lead to spikes in the robot's acceleration. 

In this section, our objective to design such a control strategy for kinematically redundant robot, i.e robots which have more degrees of freedom that required by their task. We aim to exploit that kinematic redundancy and formulate a optimization problem whose goals is to find configurations that minimize an appropriate norm of the matrix $\bm{\Gamma}(\bm{q})$ and acts cohesively with the robot's primary control task. We are particularly interested in anticipated impacts, i.e impacts which are part of the task. However, for generality we will first derive our approach with respect to a general uncertain 6d wrench and then define the case where the direction of an impact forces is known while its magnitude is uncertain.  

Let us start by defining the set of wrench perturbations as $\mathcal{W} \subset \mathbb{R}^{6}$ which contains the origin. 
\begin{equation*}
\begin{aligned}
      \mathcal{W} = \{ \Delta\bm{w}_{e} \in \mathbb{R}^{6} | \quad -\Delta\overline{\bm{w}} \leq \Delta\bm{w}_{e} \leq \Delta\overline{\bm{w}} \}
\end{aligned}
\end{equation*}
We can consequently define the set of possible instantaneous accelerations
\begin{equation*}
\begin{aligned}
      \mathcal{Y} = \{ \bnudt \in \mathbb{R}^{n_j} | \quad \bnudt = \bnudt^{*} + \bm{M}^{-1}(\q)\jacob^{T} \Delta\bm{w}_{e} \\ 
      \forall  \Delta\bm{w}_{e} \in \mathcal{W} \}
\end{aligned}
\end{equation*}
Indeed, if $\Delta \bm{w}_e = \bm{0}$ then the system acceleration is equal to the nominal one. 
Note that $\bm{\Gamma}$ is a function of the configuration $\q$, it is then possible to pose the following optimization problem. 
% the min max problem
\begin{equation}
\begin{aligned}
\min_{\q}\max_{\Delta\bm{w}_{e} \in \mathcal{W}} \quad & || \Delta \bnudt|| = \Delta\bm{w}_{e}^{T}\bm{\Gamma}(\q)^{T}\bm{\Gamma}(\q)\Delta\bm{w}_{e} \\
\end{aligned}
\label{eq:opt1}
\end{equation}
The optimization problem defined in Eq.~(\ref{eq:opt1}) has the objective of finding robot configurations that instantly minimize the norm of the worst case deviation for robot acceleration $\bnudt$ from its nominal value $\bnudt^{*}$, due to mismatch in the contact wrench. 

Naturally, a robot will have a main goal that it is tasked to achieve, and in general the configuration resulting from optimization problem in Eq.~(\ref{eq:opt1}) will not be consistent with the robot original task. In the following, we will reformulate the problem in Eq.~(\ref{eq:opt1}) within the context of operational space formulation as a secondary task. The operational space control formulation, also referred to as task space control, was first proposed in \cite{1087068}. This formulation presents a general approach to control a robot's task space, for example, controlling the pose of an End Effector (EE) of a robotic arm. 

Consider the following task kinematics described at the acceleration level
\begin{equation}
    \bnudt_t = \jacob \bnudt + \jacobdt
    \label{eq:task_kin}
\end{equation}
Where, $\bnudt_t \in \mathbb{R}^{m}$ represents the robot task, e.g the acceleration of the EE and assume that $m < n_j$ which means that the robot is kinematically redundant for the task. The task jacobian is given by $\jacob$. Now suppose, we would like to impose an acceleration $\bnudt_{t}^{*}$ to the robot task variables, where  $\bnudt_{t}^{*}$ represents a virtual control input, for example a proportional and damping controller (PD controller) and a feed-forward acceleration.
\begin{equation}
    \bnudt_{t}^{*} = \bnudt_{t}^{\text{ff}} + \bm{K}_{p}\bm{e}_p + \bm{K}_{v}\bm{e}_v
    \label{main_task}
\end{equation}
One can then compute the corresponding joint space accelerations 
\begin{equation}
    \bnudt^{*} = \jacob_{W}^{\dagger}(\bnudt_{t}^{*} - \jacobdt) + \bm{P}(\bm{q})\bnudt_{\text{null}}
    \label{eq:invdiffKin}
\end{equation}
where $\jacob_{W}^{\dagger}$ represents a weighted Moore-Penrose inverse, while $\bm{P}(\bm{q})$ represents the null space projector and $\bnudt_{\text{null}}$ is a preferred acceleration to be projected in the null-space of the task and acts as a secondary task. 

We will reformulate the optimization problem in Eq.~(\ref{eq:opt1}) as a secondary task to be projected in the null space of the primary task. We define an ellipsoid in the perturbed wrench space $\mathcal{W}$, where the semi-axis of the ellipsoid are encoded its kernel matrix $\bm{W}_e$ as follows
\begin{equation}
     \Delta\bm{w}_{e}^{T} \bm{W}^{-1}_{e} \Delta\bm{w}_{e} = 1
    \label{eq:paramellipsoid}
\end{equation}
where, $\bm{W}_{e} = \text{diag}(\Delta\overline{\bm{w}}^{2})$. We can then use the mapping provided in Eq.(\ref{impact_sens}) and project the ellipsoid from perturbed wrench space into the perturbed acceleration space. and we get 
\begin{equation}
    \Delta \dot{\bm{\nu}}^{T} (\bm{\Gamma} \bm{W}_e  \bm{\Gamma}^{T})^{\dagger} \Delta \dot{\bm{\nu}} = 1
    \label{eq:accellipsoid}
\end{equation}
Let $\bm{\Gamma} \bm{W}_e  \bm{\Gamma}^{T}=\bm{H}(\q)$ and consider the eigenvector decomposition of $\bm{H}(\q)$ (which always exists since $\bm{H}$ is symmetric and positive semi-definite) and denote the eigenvalues of $\bm{H}$ as $\bm{\Lambda}=\text{diag}(\lambda_1,\ldots,\lambda_{nj})$. The ellipsoid~(\ref{eq:accellipsoid}) will then have semi-axes of length $\sqrt{\lambda_i}$. One possible norm (to be minimized) is the largest eigenvalue of $\bm{H}$, $\lambda_{max}=\max(\lambda_1,\ldots,\,\lambda_n)$. This represents the worst (largest) deviations in the accelerations. Alternatively, one can replace the $\max(\cdot)$ operation with the Frobenius norm of $\bm{H}$, denoted as $|| H_{\Gamma} ||_{F}$. This is equivalent since $\bm{H}$ is symmetric and positive semi-definite. 

We can then exploit the robot's kinematic redundancy to design a virtual input $\dot{\bm{\nu}}^{*}$ which minimizes the Frobenius norm of $\bm{H}$, In particular we can attempt to minimize the Frobenius norm  in the null space of the task Jacobian. This is done as follows
\begin{equation} 
    \bm{\dot{\nu}}_{\text{null}} =  - \bm{K} \nabla_{\bm{q}} || H_{\Gamma} ||_{F} - \bm{K}_d \bm{\nu}
\end{equation}
Where $\bm{K}$ is a tunable positive definite gain matrix and $- \bm{K}_d \bm{\nu}$ represents the damping necessary to stabilize the null space dynamics.

In the case of anticipated impacts, we assume to know the direction $\bm{n} \in \mathbb{R}^{3}$ of the impact force. We then rewrite Eq.~(\ref{impact_sens}) as  
\begin{equation}
    \Delta \bnudt = \bm{M}^{-1}(\q)\jacob^{T} \bm{n} \Delta f_e
    \label{impact_sens_force}
\end{equation} 
Where, $\Delta f_e$ represents the uncertainty in the magnitude of the impact force along the direction $\bm{n}$. In this case we can just  

% focus on forces 




==> theory_simple.tex <==
\section{The Sensitivity of Inverse Dynamics Controllers to Uncertain Contact Forces}\label{sec:sens_def}
Consider the following dynamic equations of a rigid body robotic system subject to contact forces.
\begin{equation}
    \bm{M}(\q) \bnudt + \bm{h}(\q,\bnu) = \bm{G}(\q)\ip + \jacobc^{T}\bm{F}_c
    \label{eq:realdyn}
\end{equation}
where, $\q \in \mathbb{R}^{n}$ represents the robot's configuration space, while $\bnu \in \mathbb{R}^{n}$ represents the robot's joint velocities. $\bm{M}(\q) \in \mathbb{R}^{n \times n}$ is the inertia matrix, $\bm{h}(\q,\bnu) \in \mathbb{R}^{n}$ represents the gravitational and Coriolis effects. The system inputs $\ip \in \mathbb{R}^{n_u}$ are mapped to joint forces and/or torques via the input matrix $\bm{G}(\q) \in \mathbb{R}^{n \times n_u}$. Finally, we consider that the robot is in contact, where $\jacobc$ is the contact Jacobian and $\bm{F}_c$ are the contact forces. 

We are particularly interested in robotic systems which are controlled using an \emph{inverse dynamics} control strategy. The objective of an inverse dynamics controller is to impose a desired joint acceleration $\bnudt^{*} \in \mathbb{R}^{n}$ obtaining $\bnudt = \bnudt^{*}$. A standard inverse dynamics controller can be formulated as:
\begin{equation}
   \ip = \bm{G}^{-1}(\bm{M} \bnudt^{*} + \bm{h} - \bm{J}_{c}^{T}\hat{\bm{F}}_c)
   \label{eq:cntrl}
\end{equation} 
Where the dependency on the state has been removed for compactness. In Eq.~(\ref{eq:cntrl}), $\bnudt^{*}$ represent the virtual input that can constitute, for example, a desired impedance for physical interaction control. The $\hat{}$ symbol in Eq.~(\ref{eq:cntrl}) represents the contact forces at their nominal values. If a precise knowledge of the contact forces is available, i.e. $\bm{F}_c = \hat{\bm{F}}_c$, then the inverse dynamics controller will successfully linearize the system and impose the desired acceleration. However, in the real case the controller is uncertain about the contact forces, i.e. $\Delta \bm{F}_c = \bm{F} _c - \hat{\bm{F}}_c \neq \bm{0}$. Thus, the resulting instantaneous closed-loop acceleration will take the form
\begin{equation}
        \bnudt = \bnudt^{*} + \bm{M}^{-1}(\q)\jacobc^{T} \Delta \bm{F}_{c}
    \label{eq:CLdyn}
\end{equation}
We can rewrite in Eq~(\ref{eq:CLdyn}) as follows
\begin{equation}
    \Delta \bnudt = \bm{M}^{-1}(\q)\jacobc^{T} \Delta\bm{F}_{c}
    \label{impact_sens}
\end{equation} 
Where $\Delta \bnudt = \bnudt - \bnudt^{*}$, represents the deviation of the robot's acceleration from its nominal value $\bnudt^{*}$. Equation~(\ref{impact_sens}), represents the instantaneous sensitivity of the closed-loop acceleration (in closed-form) with respect to the uncertainty in the external force. We denote the sensitivity matrix by
\begin{equation}
    \label{eq:Gamma}
    \bm{\Gamma}(\q) = \bm{M}^{-1}(\q)\jacobc^{T}.
\end{equation}
Its interesting to note that the quantity $\bm{M}^{-1}(\q)\jacobc^{T}$ has a well known physical interpretation, as it maps contact forces to the robot's joint acceleration, when the robot is at rest $\bnu = \bm{0}$. However, in our derivation of $\bm{\Gamma}(\q)$, we provide a new perspective on the role of this mapping for inverse dynamics controllers in the presence of uncertainty in the contact force. In the following, we will demonstrate how to exploit this new perspective to minimize the effect of force uncertainty in particular during impacts.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Optimizing for Impact-Robust Postures}\label{sec:sens_opt}
Specifically focusing on impact events, the practical difficulties in estimating or measuring the impact forces indicate the presence of large force uncertainties over short periods of time. Equation~(\ref{impact_sens}), highlights that large force uncertainties can lead to \textbf{instantaneously} large variations in the robot acceleration and hence its state.  It was shown in \cite{9636094}, that such rapid state variations, can potentially lead to \emph{spikes} in the control commands, which are difficult to be practically realized by a robot's actuators thus degrading the controller performance. Our objective is to design a control strategy, for robots with redundant degrees of freedom, that can optimize the robot's posture for mitigating the effects of force uncertainty during impacts. 

We are particularly interested in anticipated impacts, i.e. impacts which are part of the task. We will assume the contact happens at a known location, e.g the EE of the robot, and that the direction at which the impact force acts is known as well. We will formulate an optimization problem with the goal of finding the robot configuration that minimizes a norm of the matrix $\bm{\Gamma}(\bm{q})$ while simultaneously acting cohesively with the robot's primary control tasks. For the sake of generality, we will first derive our approach with respect to a generic uncertain force (uncertain magnitude and direction) and then consider the special case where the direction of the impact force is known while its magnitude is uncertain. 

%As described in~(\ref{impact_sens}), large force uncertainties can lead to instantaneously large variations or \emph{spikes} in the robot state. It was shown in that potentially lead to spikes in the control commands, which are difficult to be realized on the system's actuators, degrading the controller performance. This motivates designing a control strategy that renders the robot insensitive to impacts, i.e. the uncertainty in the impact forces does not lead to spikes in the robot's state. 

%In this section, our objective to design such a control strategy for kinematically redundant robot, i.e. robots which have more degrees of freedom than the ones required by their task. We aim to exploit  kinematic redundancy and formulate a optimization problem whose goals is to find robot configurations that minimize an appropriate norm of the matrix $\bm{\Gamma}(\bm{q})$ and also act cohesively with the robot's primary control task. 

%In the following developments we will assume the contact happen at a known location, e.g the EE of the robot. Moreover, we are particularly interested in anticipated impacts, i.e. impacts which are part of the task. This implies that the the direction at which the impact force acts is also known. However, for generality we will first derive our approach with respect to a generic uncertain force and then define the case where the direction of the impact force is known while its magnitude is uncertain.  
Consider the following set $\mathcal{F}$ of contact force perturbations defined as
\begin{equation*}
\begin{aligned}
      \mathcal{F} = \{ \Delta\bm{F}_c \in \mathbb{R}^{3} \;| \; -\Delta\overline{\bm{F}} \leq \Delta\bm{F}_c \leq \Delta\overline{\bm{F}} \}.
\end{aligned}
\end{equation*}
Where $\Delta\overline{\bm{F}} \in \mathbb{R}^{3}$ represents the bounds on the contact force uncertainty. Consequently, the set $\mathcal{Y}$ of joint acceleration perturbations is defined as 
\begin{equation*}
\begin{aligned}
      \mathcal{Y} = \{ \bnudt \in \mathbb{R}^{n} \;| \; \bnudt = \bnudt^{*} + \bm{M}^{-1}(\q)\jacobc^{T} \Delta\bm{F}_c \\ 
      \forall  \Delta\bm{F}_c \in \mathcal{F} \}
\end{aligned}
\end{equation*}
Indeed, if $\Delta \bm{F}_c = \bm{0}$ then the robot's acceleration is equal to the nominal one. 

Since the matrix $\bm{\Gamma}$ is a function of the robot's configuration $\q$, it is then possible to pose the following optimization problem: 
% the min max problem
\begin{equation}
\begin{aligned}
\min_{\q}\max_{\Delta\bm{F}_{c} \in \mathcal{F}} \quad & || \Delta \bnudt||^{2} \\
\end{aligned}
\label{eq:opt1}
\end{equation}
The optimization problem defined in~(\ref{eq:opt1}) has the objective of finding robot configurations that instantly minimize the norm of the worst case deviation for robot acceleration $\bnudt$ from its nominal value $\bnudt^{*}$, due to mismatch in the contact force. In general the configuration resulting from optimization problem in~(\ref{eq:opt1}) will not be consistent with the robot original task. 

In the following, we will reformulate the problem in~(\ref{eq:opt1}) within the context of the operational space formulation \cite{1087068} as a secondary task. This formulation presents a general approach to control a robot's task space, e.g. controlling the pose of an EE of a robotic arm. 

Suppose that we would like to impose an acceleration $\bnudt_{t}^{*}$ to the robot task variables, where  $\bnudt_{t}^{*}$ represents a virtual control input, e.g. a desired EE impedance, and consider the task kinematics described at the acceleration level as
\begin{equation}
    \bnudt_t = \jacob \bnudt + \jacobdt,
    \label{eq:task_kin}
\end{equation}
where $\jacob$ is the task Jacobian and $\bnudt_t \in \mathbb{R}^{m}$ represents the robot task, e.g. an acceleration of the EE. Note that we are interested in kinematically redundant robots where $m < n$.
The corresponding desired joint space accelerations are given by
\begin{equation}
    \bnudt^{*} = \jacob_{W}^{\dagger}(\bnudt_{t}^{*} - \jacobdt) + \bm{P}(\bm{q})\bnudt_{\text{null}}
    \label{eq:invdiffKin}
\end{equation}
where $\jacob_{W}^{\dagger}$ represents a weighted Moore-Penrose inverse, while $\bm{P}(\bm{q})$ represents the null space projector and $\bnudt_{\text{null}}$ is a preferred acceleration to be projected in the null-space of the task and acts as a secondary task. 

We will reformulate the optimization problem in~(\ref{eq:opt1}) as a secondary task which is to be projected in the null space of the primary task. Consider the following set $\mathcal{E}_f \subset \mathcal{F}$ defined as 
\begin{equation*}
\begin{aligned}
      \mathcal{E}_f = \{ \Delta\bm{F}_c \in \mathcal{F} \;| \; \Delta\bm{F}_{c}^{T} \bm{W}^{-1}_{c} \Delta\bm{F}_{c} \leq 1 \}.
\end{aligned}
\end{equation*}
The set $ \mathcal{E}_f$ represents an ellipsoid in the perturbed force space $\mathcal{F}$, where the semi-axis of the ellipsoid are encoded by its kernel matrix $\bm{W}_{c} = \text{diag}(\Delta\overline{\bm{F}}^{2})$. We can then use the mapping provided in~(\ref{impact_sens}) and project the ellipsoid from the force space into the acceleration space. 
\begin{equation}
    \Delta \dot{\bm{\nu}}^{T} (\bm{\Gamma} \bm{W}_c  \bm{\Gamma}^{T})^{\dagger} \Delta \dot{\bm{\nu}} \leq 1
    \label{eq:accellipsoid}
\end{equation}

Let $\bm{\Gamma} \bm{W}_c  \bm{\Gamma}^{T}=:\bm{H}_{\Gamma}(\q)$ and consider the Frobenius norm as one possible norm to be minimized. Since $\bm{H}_{\Gamma}(\q)$ is a positive semi-definite matrix, minimizing the Frobenius norm is equivalent to minimizing the largest semi-axis of the acceleration ellipsoid, which represents the worst case deviations in the accelerations. 
%consider the eigenvector decomposition of $\bm{H}(\q)$ (which always exists since $\bm{H}$ is symmetric and positive semi-definite) and denote the eigenvalues of $\bm{H}(\q)$ as $\bm{\Lambda}=\text{diag}(\lambda_1,\ldots,\lambda_{nj})$. The ellipsoid~(\ref{eq:accellipsoid}) will then have semi-axes of length $\sqrt{\lambda_i}$. One possible norm (to be minimized) is the largest eigenvalue of $\bm{H}(\q)$, $\lambda_{max}=\max(\lambda_1,\ldots,\,\lambda_n)$. This represents the worst (largest) deviations in the accelerations. Alternatively, one can replace the $\max(\cdot)$ operation with the Frobenius norm of $\bm{H}(\q)$, denoted as $|| H_{\Gamma} ||_{F}$. This is equivalent since $\bm{H}(\q)$ is symmetric and positive semi-definite. 

We can then exploit the robot's kinematic redundancy to design a virtual input $\dot{\bm{\nu}}^{*}$ which minimizes the Frobenius norm of $\bm{H}_{\Gamma}(\q)$, In particular we can attempt to minimize the Frobenius norm  in the null space of the task Jacobian. This can be achieved as follows
\begin{equation} 
    \bm{\dot{\nu}}_{\text{null}} =  - \bm{K} \nabla_{\bm{q}} || \bm{H}_{\Gamma} ||_{F} - \bm{K}_d \bm{\nu}
\end{equation}
Where $\bm{K}$ is a tunable positive definite gain matrix and $- \bm{K}_d \bm{\nu}$ represents the damping necessary to stabilize the null space dynamics.

In the case of anticipated impacts, we assume to know the unit vector representing the direction $\bm{n} \in \mathbb{R}^{3}$ of the impact force. We then rewrite~(\ref{impact_sens}) as  
\begin{equation}
    \Delta \bnudt = \bm{M}^{-1}(\q)\jacob^{T} \bm{n} \Delta f_c
    \label{impact_sens_force}
\end{equation} 
Where, $\Delta f_c$ represents the uncertainty in the magnitude of the impact force along the direction $\bm{n}$. In this case, the sensitivity matrix will include the direction of the force, $\bm{\Gamma}(\q) = \bm{M}^{-1}(\q)\jacob^{T} \bm{n}$. As outlined earlier, we can then compute the perturbed acceleration ellipsoid as in~(\ref{eq:accellipsoid}).

% focus on forces 



